Machine Learning for Spectrum Sharing: A Survey

The 5th generation (5G) of wireless systems is being deployed with the aim to provide many sets of wireless communication services, such as low data rates for a massive amount of devices, broadband, low latency, and industrial wireless access. Such an aim is even more complex in the next generation wireless systems (6G) where wireless connectivity is expected to serve any connected intelligent unit, such as software robots and humans interacting in the metaverse, autonomous vehicles, drones, trains, or smart sensors monitoring cities, buildings, and the environment. Because of the wireless devices will be orders of magnitude denser than in 5G cellular systems, and because of their complex quality of service requirements, the access to the wireless spectrum will have to be appropriately shared to avoid congestion, poor quality of service, or unsatisfactory communication delays. Spectrum sharing methods have been the objective of intense study through model-based approaches, such as optimization or game theories. However, these methods may fail when facing the complexity of the communication environments in 5G, 6G, and beyond. Recently, there has been significant interest in the application and development of data-driven methods, namely machine learning methods, to handle the complex operation of spectrum sharing. In this survey, we provide a complete overview of the state-of-theart of machine learning for spectrum sharing. First, we map the most prominent methods that we encounter in spectrum sharing. Then, we show how these machine learning methods are applied to the numerous dimensions and sub-problems of spectrum sharing, such as spectrum sensing, spectrum allocation, spectrum access, and spectrum handoff. We also highlight several open questions and future trends.

==> NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> Sections/Process/spectrumsharingprocess.tex <==
%\section{Spectrum Sharing Process}\label{Sec:Process}

%Spectrum sharing can be performed either in a centralized \cite{V.Brik2005,Carroll2012,Deb2009,Miao2016} or distributed manner \cite{Lin2010,Shamsoshoara2019,Chang2019,Naparstek2019}. 

%Spectrum sharing can be performed either in a centralized  or distributed manner. The former is characterized by a central unity, often called spectrum  server, which is responsible for optimizing the spectrum usage among all users. %This approach is suitable to solve the hidden terminal problem on \acp{CRN} \cite{Carroll2012} and to facilitate the sharing of television white spaces \cite{Deb2009}.
%In the latter, all network users participate in the spectrum optimization process. It is a more practical solution for high spectral demand since the computational complexity at the central unity increases with the number of spectrum requests \cite{Lin2010}. 
%
%In a spectrum sharing scenario, the coexistence of different wireless systems are provided by four  mechanisms:
%\begin{enumerate}
%	\item \textit{Spectrum sensing}: in this mechanism, signal features are extracted from the environment to determine the radio frequency occupancy condition, i.e., which channels are in use and which ones are free.
%	\item \textit{Spectrum allocation}: receives the channel characterization from sensing mechanism or directly from the environment in case of frequency planing. The main goal is to assign users on available channels for data transmission.
%	\item \textit{Spectrum access}: the user assignment is used in this stage to provide channel access for allocated users in order to guarantee the data transmission. 
%	\item \textit{Spectrum handoff}: responsible for user channel switching whenever necessary. It sends a request to the spectrum allocation mechanism to check and to assign a new channel to the user so it can continue to access the medium sending its data.
%\end{enumerate}
%	
%This relationship between the four spectrum sharing mechanisms is showed in Figure \ref{fig:spectrumsharing}.
%
%\begin{figure}
%	{\includegraphics[width=0.5\textwidth]{figs/SS/spectrum_sharing_figure.pdf}}
%	\caption{Spectrum sharing example scenario.}
%	\label{fig:spectrumsharingscenario}
%\end{figure}




%In a spectrum sharing scenario, the coexistence of different wireless systems are provided by the following  mechanisms: spectrum sensing and geolocation databases \cite{Park2014}.  The other spectrum sharing steps include spectrum allocation, spectrum access and spectrum handoff \cite{Hu2018}.} 

%\cite{Hu2018}
%The core idea of CR is to realize spectrum sharing through dynamic spectrum access, and the implication of spectrum
%sharing is that SUs can use the idle spectrum of PUs, but only if they cannot interfere with the communication of PUs. Typically, spectrum sharing includes four steps,
%
%1) Spectrum sensing: Spectrum sensing is the first step of spectrum sharing, which is the fundamental to ensure PUs from interference, to complete spectrum sharing, to improve spectrum utilization, and to realize various CR applications. SUs continuously detect the frequency bands that are being used by PUs in multi-dimensional space (such as time domain, spatial domain, frequency domain, etc.). Spectrum sensing is utilized to detect whether a PU appears and to determine if the spectrum hole is available. Therefore, the accurate perception of spectrum
%holes is the first step in spectrum sharing.
%
%2) Spectrum allocation: Spectrum allocation is based on the availability of spectrum holes and distributes the spectrum to SUs. Since the number of spectrum holes is not fixed, SUs need to use them through competition while the QoS of SUs are different. Therefore, the spectrum holes have to be used fairly and efficiently. The key of spectrum
%allocation is to design efficient spectrum allocation algorithms and rules, which can improve the efficiency of spectrum utilization in the case of conflict minimization or conflict-free, preferably as close to the optimal
%target as possible.
%
%3) Spectrum access: PU has the priority access rights of the frequency band, while the SU as subordinate relationship access it. Therefore, spectrum access requires an efficient access algorithm to coordinate multiple SUs access spectrum holes, avoiding conflicts between PUs and SUs.
%
%4) Spectrum handoff: SU must switch to the appropriate spectrum when one of the following three situations occurs. First of all, when the SU using a current spectrum hole, the appearance of PU will cause collisions between them, thus SU must quit this frequency band, and then switch to the other spectrum holes for communication. Secondly,
%when the geographical location of the SUs changes, while the PU’s geographical location does not change, the optional spectrum holes for the SUs will be different, and they need to switch to the appropriate frequency band. Finally, when the frequency bands used by SUs cannot meet their communication requirements, they must switch to other frequency band that can meet their communication needs.
\section{Spectrum Sensing}\label{Sec:Sensing}
\input{Sections/Process/sensing.tex}

\section{Spectrum Allocation}\label{Sec:Allocation}
\input{Sections/Process/allocation.tex}

\section{Spectrum Access}\label{Sec:Access}
\input{Sections/Process/access.tex}

 \section{Spectrum Handoff}\label{Sec:Handoff} 
\input{Sections/Process/handoof.tex}


 



 

 
%\input{Sections/Process/spectrumsharingtable.tex}


==> Sections/Process/spectrumsharingtable.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h!]
	\caption{Table Summary.}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Work}  & \multicolumn{4}{c|}{Spectrum Sharing}                                       & \multirow{2}{*}{Scenario} \\ \cline{2-5}
		& Spectrum Sensing & Spectrum Allocation & Spectrum Access & Spectrum Handoff &                           \\ \hline
		\cite{Zhang2019} &   $\checkmark$               &       -              &    -              &  -                &  \ac{CRN} single \ac{PU} and \ac{SU}            \\ 
		\cite{Handouf2018} &        -          & $\checkmark$                    &    -             &  -                &  \ac{CRN} multiple \acp{SU}                         \\ \hline
	\end{tabular}
\end{table}
